The Optimal Paper Moebius Band

In this paper we prove that a smooth embedded paper Moebius band must have aspect ratio greater than $\sqrt 3$. We also prove that any sequence of smooth embedded paper Moebius bands whose aspect ratio converges to $\sqrt 3$ must converge, up to isometry, to the famous triangular Moebius band. These results answer the minimum aspect ratio question discussed by W. Wunderlich in 1962 and prove the more specific conjecture of B Halpern and C. Weaver from 1977.

==> 4bends.tex <==

\section{Appendix: Proof of Lemma \ref{mc}}
\label{bends}

We give a self-contained proof of Lemma \ref{mc}.
Let $S^2$ be the unit $2$-sphere.
The {\it Gauss map\/}, which is well defined and
smooth on any
simply-connected subset of $\Omega$,
associates to each
point $p \in \Omega$ a unit normal vector $n_p \in S^2$.
Let $dn_p$ be the differential
of the Gauss map at $p$.
Since the curvature $\Omega$ is $0$ everywhere,
$dn_p$ has a nontrivial kernel. The point $p$
has nonzero {\it mean curvature\/}
if and only if $dn_p$ has nontrivial image.

Let $U$ be as in Lemma \ref{mc}, the subset of
$\Omega^o$ with nonzero mean curvature.
Let $p \to n_p$ be a local choice
of the
Gauss map. We
can rotate and translate so that
near the origin $U$ is the graph of a function
\begin{equation}
  \label{norm}
F(x,y)=Cy^2 + {\rm higher\ order\ terms\/}.
\end{equation}
Here $C>0$ is some constant.
The normal vector at the origin is $n_0=(0,0,1)$.
The vector $v_0=(1,0,0)$ lies in the kernel of $dn_0$.
Let $w_0=(0,1,0)$.
Let $\Pi_0$ be the plane spanned by $w_0$ and $n_0$.
The image of $\Pi_0 \cap U$ under
the Gauss map is (near $n_0$)
a smooth regular curve tangent to
$ w_0$ at $n_0$.  The sign depends on
the choice of local Gauss map.

Working locally,
we have three smooth vectorfields:
\begin{equation}
p \to n_p, \hskip 30 pt p \to v_p, \hskip 30 pt
p \to w_p=v_p \times n_p.
\end{equation}
Here $v_p$ is the kernel of $dn_p$ and $\times$ denote the cross product.
Let $\Pi_p$ be the plane through $p$ and spanned by $w_p$ and $n_p$.
From our analysis of the special case, and from symmetry,
the image of $\Pi_p \cap U$ under the Gauss map is
(near $n_p$) a
smooth regular curve tangent to $ w_p$ at $n_p$.
The {\it asymptotic curves\/} are the smooth curves
everywhere tangent to the $v$ vector field.

\begin{lemma}
  The asymptotic curves are line segments.
\end{lemma}

\startproof
Let $\gamma$ be an asymptotic curve.
The Gauss map is constant along $\gamma$.
Each point in $\gamma$ has a
small neighborhood $V$ which is
foliated by asymptotic curves
that transversely intersect each plane $\Pi_p$
when $p \in \gamma \cap V$.
Hence the image of $V$ under the Gauss map
equals the image of $\Pi_p \cap V$ under the Gauss map.
This latter image is a smooth regular curve tangent
to $w_p$ at $n_p$.
Since this is true for
all $p \in \gamma \cap V$
and since $n_p$ is constant along $\gamma$, 
$w_p$ is constant along $\gamma$.
Hence $v_p$ is constant along $\gamma$. Hence
$\gamma$ is a line segment.
\endproof



The nonzero mean curvature implies
that $\gamma$ is the unique line segment through
any of its interior points.  
We first rule out the possibility that
$\gamma$ reaches $\partial U$ before it reaches
$\partial \Omega$.
Assume for the sake of contradiction that this happens.
We normalize as in Equation \ref{norm}.

We now allow ourselves the liberty of
dilating our surface.  This dilation preserves
all the properties we have discussed above.
By focusing on a point of $\gamma$ sufficiently
close to $\partial U$ and
dilating, we arrange the following:
\begin{itemize}
  \item A neighborhood $\cal V$ of
$\Omega^o$ is the graph of a function over 
the disk of radius $3$ centered at the origin.
\item  Given $p \in \cal V$ let $p'$ be the projection of $p$ to the
  $XY$-plane.
  We have $|p_1'-p_2'|>(2/3)|p_1-p_2|$ for all $p_1,p_2 \in \cal V$.
\item $\gamma \subset U$ contains the arc connecting
  $(0,0,0)$ to $(3,0,0)$, but $(0,0,0) \not \in U$.
  \end{itemize}

  Let $a \in (0,3)$.
  At $(a,0,0)$ we have
$v_a=(1,0,0)$ and $w_a=(0,1,0)$ and $n_a=(0,0,1)$.
Let $\Pi_a$ be the plane $\{X=a\}$.
Near $(a,0,0)$, the intersection
$U_a=U \cap \Pi_a$ is a smooth curve tangent to
$w_a$ at $(a,0,0)$.

Let $\zeta=(1,0,0)$.
    Fix $\delta>0$.  By continuity and compactness,
    the asymptotic curves through points of
    $U_{1}$ sufficiently near
    $\zeta$ contain line segments connecting
    points on $U_{2}$ to points on $U_{\delta}$.
    Call these {\it connectors\/}.
        There exists a canonical map
    $\Phi_{\delta}: U_{1} \to U_{\delta}$
    defined in a neighborhood of $\zeta$:
    The points $q \in U_{1}$ and
    $\Phi_{\delta}(q) \in U_{\delta}$ lie in the same connector.
    
\begin{lemma}
  \label{expand}
  $\Phi_{\delta}$ expands  distances by less than
  a factor of $3$.
\end{lemma}

\startproof
Let $\ell_1$ and $\ell_2$ be two connectors.
Let $a_j=\ell_j \cap U_1$.
Let $b_j = \ell_j \cap U_{\delta}$.
For any set $S$
let $S'$ be the projection of $S$ to $\R^2$.
We have the bounds
$$\frac{|a_1'-a_2'|}{|a_1-a_2|},
\frac{|b_1'-b_2'|}{|b_1-b_2|} \in \bigg[\frac{2}{3},1\bigg],
\hskip 30 pt
\frac{|a_j'-b_j'|}{{\rm length\/}(\ell_j')}<2.
$$
Geometrically, $a_j'$ is very nearly the midpoint of $\ell_j'$
and $b_j'$ is the closer of the two endpoints.
Since $\ell_1'$ and $\ell_2'$ are planar and disjoint, our last inequality
(and essentially a similar-triangles argument) gives
$|b_1'-b_2'|/|a_1'-a_2'|<2.$
Putting everything together, we have
$|b_1-b_2|/|a_1-a_2|<3$.
\endproof

Fix $\epsilon>0$.
The mean curvature along $U_{\delta}$ tends to
$0$ as $\delta \to 0$.
If we choose $\delta$ sufficiently
small then the Gauss map expands distances
along $U_{\delta}$ in a neighborhood of
$(\delta,0,0)$ by a factor of less than
$\epsilon$.  Combining
Lemma \ref{expand} and the fact that
$n_q=n_{\Phi_{\delta}(q)}$, we see that
the Gauss map expands
distances by at most a factor of
$3\epsilon$ along $U_{1}$ in a small
neighborhood of $\zeta$.
Since $\epsilon$ is arbitrary,
$w_1 \in {\rm ker\/}(dn_{\zeta})$.  But
$v_1 \in {\rm ker\/}(dn_{\zeta})$ by definition.  Hence
$dn_{\zeta}$ is the trivial map.
The contradicts the fact that $\zeta \in U$.

Now we know that the interior of $\gamma$ lies in
$U$.  Next, we show that the mean curvature cannot
vanish at an endpoint of $\gamma$.  As discussed
in \S \ref{interpret},  there is some $\epsilon>0$ so that
$I$ has a smooth extension to the fatter open Moebius band
$M^{\epsilon}_{\lambda}$ described in Equation \ref{fatten}.
If we knew that this smooth extension was also an
isometric embedding,
we could just use our previous
argument exactly as is.  (Compare the discussion
in \S \ref{interpret}.)
But, even if
the extension is not an isometric map, we can still
use the essentially the same argument.
This time our open disk of radius $3$ is divided into
two sides, a lightly shaded
{\it familiar side\/} consisting of projections of points of
$\Omega$ and a darkly shaded {\it mystery side\/}
consisting of projections of points of
$I(M_{\lambda}^{\epsilon})-I(M_{\lambda})$.
The common boundary of these regions is curve,
transverse to the $x$-axis, which is a projection
of $I(\partial M_{\lambda})$.  Figure 5 shows what
we are taking about.


\begin{center}
\resizebox{!}{1.41in}{\includegraphics{Pix/divider.eps}}
\newline
{\bf Figure 5:\/} The connectors lie on the familiar side.
\end{center}

In the argument above, we can take the connectors to
all lie in the familiar side, as shown in Figure 5.  Then
we can run exactly the same argument without
ever entering into the mystery side. We then
get the same contradiction as above.  Hence the
mean curvature does not vanish at an endpoint.

This completes the proof of Lemma \ref{mc}.

\newpage







  




